Optimizing XML querying using type-based document projection

XML data projection (or pruning) is a natural optimization for main memory query engines: given a query Q over a document D, the subtrees of D that are not necessary to evaluate Q are pruned, thus producing a smaller document D'; the query Q is then executed on D', hence avoiding to allocate and process nodes that will never be reached by Q. In this article, we propose a new approach, based on types, that greatly improves current solutions. Besides providing comparable or greater precision and far lesser pruning overhead, our solution ---unlike current approaches--- takes into account backward axes, predicates, and can be applied to multiple queries rather than just to single ones. A side contribution is a new type system for XPath able to handle backward axes. The soundness of our approach is formally proved. Furthermore, we prove that the approach is also complete (i.e., yields the best possible type-driven pruning) for a relevant class of queries and Schemas. We further validate our approach using the XMark and XPathMark benchmarks and show that pruning not only improves the main memory query engine's performances (as expected) but also those of state of the art native XML databases.

==> abstract.tex <==
XML data projection (or pruning) is  a natural optimization for
main memory query engines: given a query $Q$ over a document $D$, 
the subtrees of $D$ that are not necessary to evaluate $Q$ are 
pruned, thus producing a smaller document $D'$; the query $Q$ is 
then executed on $D'$, hence avoiding to allocate and process nodes 
that will never be reached by $Q$.

   In this article, we propose a new approach, based on types, that
greatly improves current solutions. Besides providing comparable
or greater precision and far lesser pruning overhead, our 
solution ---unlike current approaches--- takes into account backward axes,
predicates, and can be applied to multiple queries rather than just to
single ones. A side contribution is a new type system for XPath
able to handle backward axes.
   The soundness of our approach is formally proved. Furthermore,
we prove that the approach is also complete (i.e., yields the best
possible type-driven pruning) for a relevant class of queries and
Schemas. We further validate our approach using the XMark and
XPathMark benchmarks and show that pruning not only improves the
main memory query engine's performances  (as expected) but also 
those  of state of the art native XML databases.


==> conclusion.tex <==
\section{Conclusion and future work}
\label{sec:conclusion}
%%\kim{ Shortcoming mentioned by the reviewers of VLDB06 version:
%%   1 st reviewer: Can you apply to XML Schema (yes formally treated), Is the approach still
%%   efficient for more aggressive main memory engine (Saxon) (yes).
%%   2nd reviewer: Reviewer two simply stated that he didn't believe in
%%   main-memory XML querying. We showed in the experiment that type
%%   projection can also improve the situation for indexing XML engine
%%   such as MonetDB.
%%   3rd reviewer: asked for a better comparison with Marian and
%%   Simeon's work and also stated that applying 'backward axes'
%%   rewriting to their work would do the trick.
%%   I gave a full comparison (for all 20 XMark queries) in terms of
%%   pruning precision, since it's the only thing we can compare with.
%%   I also discussed at the end of the comparison with related work why
%%   rewriting backward axes into forward wasn't always possible and
%%   even if possible would yield an exponential blow-up in the size of
%%   the query and introduce feature such as predicates and
%%   descendant-or-self which hinders the precisions of Marian and
%%   Simeon's technique}
%

   Our experiments show the clear advantages of applying our
   optimisation technique to query XML documents, and the
   characteristics of our solution make it profitable in all
   application scenarios. We discussed several aspects for which our
   approach improves the state of the art: for performances (better
   pruning, more
   speedup, less memory consumption), for the analysis techniques
   (linear pruning time, negligible memory and time consumption),
   for its generality (handling of all axes and of predicates), and, last
   but not least, for the formal foundation it provides (correctness
   formally proved, limits of the approach formally stated).
   
   The present work extends and  improves  the preliminary version presented
   at VLDB 2006 \cite{BCCN06} in several aspects. From  a formal point of view,
   the use of regular tree grammars as schema model makes the
   technique applicable to the various kind of schemas currently in
   use. Furthermore, the closure properties that we proved ensure that
   type-based projection is at most as expensive as validation for a
   given class of schema language. We also handle a richer set of
   queries formally (in particular we handle nested
   predicates in XPath$^\ell$) and took special care to document how
   to encode or approximate several important XPath idioms that were
   lacking from the formal presentation. On a practical level, we have
   validated our approach against state of the art query engines, using
   realistic queries and data sets. In particular, not only did we
   test against an efficient main memory query engine (Saxon) but also
   demonstrated that our approach can be used to improve, sometimes by a double digit factor, the
   performances of an already very optimized disk-based XML database
   such as MonetDB/XQuery.

   
   Future work will be pursued both at a formal and practical level.
   At a formal level, one of the main shortcoming of our approach is
   its reliance on XPath syntax. Indeed, even though we managed to
   isolate a fragment of XPath that we could formally reason with, it
   still leaves us with a syntax-directed approach. The problem with
   this is twofold. First, it makes the proofs and the specification
   of algorithms quite tedious and unnecessarily intricate. Second and
   more importantly, our pruning inference algorithm might yield
   different type projectors depending on the syntax of the original
   query. For future work, we would like to tackle a semantic based
   approach. In particular it seems worthwhile to consider more
   theoretically sound formalisms for tree queries such as, for instance, MSO
   formula or tree automata. The latter in particular would allow us
   to reuse our pruning algorithm for pattern-matching based languages
   (such as the \cduce{} language \cite{cduce} and its pattern-based query language
   \cql~\cite{cedricthesis,BCM05,Cas05a}). It is also known that tree-automata
   (as well as MSO formula) have better closure properties than
   XPath expressions and support fine-grained set-theoretic operations
   (intersection, union, complement) that have been used with success
   to devise very precise type-systems for XML \cite{FCB08}. 

   At a practical level we would like to see a tighter integration
   between document-projection and query engines.
   Firstly, although quite crude, our experiments show that even a
   carefully designed indexed system such as MonetDB can benefit from
   document pruning. It seems interesting to develop further such preliminary results    and   design  a projection aware XML index. In other words we would like to be able to equip any native XML query engine optimizer  with a type-projector component. In
   particular, one could think of an index consisting of the original
   document together with its projected versions. Textual data could be shared between the main document and the
   projected ones which would merely become a projected view of the
   tree structure of the document. We make the hypothesis that the
   overhead of such pruned tree structures would be quite small compared
   to the size of an XML index while providing significant speed-up in
   query answering time.

   Secondly, coupling our projection algorithm with early query
   answering techniques would allow us to achieve further pruning,
   especially when runtime conditions are involved. For instance we
   could use our type-inference algorithm to determine on what type of
   elements a given built-in function is applied to; for instance in an expression
   such as\\
   \centerline{\texttt{contains(.//*, "foo")}.}
   This
   information could then be used at loading time to discard
   elements that do not match the predicate.



==> extother.tex <==
%% extensions to other typing policies
\section{Extension to other typing policies}
\label{sec:extother}
\subsection{Handling  un-typed documents}
Although the usage of schema is  being more and more wide-spread, it  still is
interesting to see how to perform type-based projection
in an untyped world. A first, rather blunt, approach is to consider a
fixed corpus of un-typed documents. For such sets of documents it is
possible to \emph{infer} a \dtd{}. For instance, Bex \emph{et. al.}
 propose several automata-based methods to
infer \dtd{}s \cite{bex06} and even XMLSchemas (\cite{bex07,bex08}).
Once a schema is inferred, our technique can be applied as-is.


More interestingly, this untyped problem can be reduced to a precise
typing problem. Indeed, an un-typed document is nothing but a document
of type $(\{ X \}, \{ X \rightarrow \Any{}\})$. If we apply the type
inference-algorithm of Section~\ref{ssec:typeinf} to such an input
type, then the result would be $(\{ X \}, \{ X
\rightarrow \Any{}\})$ itself (meaning that the nodes selected by the
query have type $\Any{}$). Therefore in this case, since none of the
intermediary steps of the query results in an empty-type, the
type-projector inference algorithm of Section~\ref{ssec:typrojinf} cannot
remove any rule from the input type which remains $(\{ X \}, \{ X
\rightarrow \Any{}\})$: the input document cannot be
pruned. However, even though the input type does not contain any meaningful
information, the query itself might. Imagine a query
``\XPATH{//a/b}''. It is easy to deduce, by  a simple examination of the query a
projector which keeps only ``b'' nodes occurring below ``a''-nodes.
While the solution in this case is straightforward, solving this problem in general is a tricky issue. The solution for a
forward fragment of XPath can be found in the last author's PhD.\ thesis (see
Chapter~7 of \cite{kimthesis}). Let us briefly outline it on our example.
The first issue is the representation
of types. For such precise algorithms, regular tree grammars are not
well suited. Indeed instead of the type 
$(\{ X \}, \{ X \rightarrow \Any{}\})$, it is more desirable to have a
type $(\{X\}, E )$ where $E$ is the set of rules:
$$
\{ X\rightarrow String,~~X\rightarrow \_[ ~X*~ ] \}
$$
where $\_$ denotes the set of all possible tree labels. Then the
result of a query \XPATH{//a/b} applied to a a tree of the above type (i.e., any XML tree) would be the type projector:
$$
\{ X\rightarrow \_[ ~X+~ ],~X\rightarrow a[ ~B+~ ],~B\rightarrow b[~Y*~],~
Y\rightarrow \String,~ Y\rightarrow \_[ ~Y*~ ] \}
$$
%\beppe{The following paraph is not clear, it should be rewritten}
%\kim{done}

Note that this type-projector is non-deterministic top-down. It
matches (and therefore keeps) any subtree $t$ if and only if there is
a subtree $t'$ of $t$ with tag ``a'' which itself has a non-empty
sequence of children tagged ``b''. Nodes that are children of an ``a''
node but whose tag is not ``b'' do not have any interpretation and
therefore are discarded. 

% First, note that from this projector, the only way to keep a leaf in
% the input document (node typed with $Y$ and $B$), then an ancestor of
% the leaf (or the leaf itself) must be a ``b''-node. Then, note that a 
% ``b''-node can only be below an ``a''-node, and that the latter can
% occur anywhere in the input document. Therefore, the only nodes in an
% input document which have an interpretation ---and therefore are kept by
% the type projector--- are exactly the
% ``b''-nodes (and their content) which are below ``a''-nodes, and all
% their ancestors. For instance nodes occurring below an ``a'' which are
% not labelled ``b'' are not matched by any rule, and therefore can be safely
% removed.

In \cite{kimthesis}, in order to achieve such a precise typing, the inference algorithm makes a heavy use of \cduce's
type algebra (see~\cite{FCB08}) in particular of intersection and
negation types. Also note that the projector above is not obtained
by erasing some of the rules of the original type but by the mean of
set theoretic operations . In fact, 
three new rules were created and intuitively
they were obtained by intersecting the initial
``$X\rightarrow \_[ ~X*~ ]$'' rules with a type ``$a[ ~B+ ]$'' which
is the constraint
represented by the XPath query. Note also that contrary to our
approach where new rules are only erasures of existing ones (of which
there only exists a finite number), special care must
be taken to not introduce infinitely many refined rules or, said
differently, in this
context even guarantying the termination of the algorithm is a very
delicate issue.

\subsection{Using regular tree languages as schemas}
\label{ssec:regularproj}
While our formal development remains in the very general case of
regular tree grammars, our implementation only focuses on \dtd{}s. The main reason is that 
for \dtd{}s pruning is efficient memory-wise. For regular tree languages
instead, validation (and pruning) may need to visit the whole tree before
deciding which node to prune. At first, it seems that this completely
defeats the purpose of pruning, but we argue that pruning can still be
of practical use in these cases.

Indeed, a way of addressing this problem is to temporarily store 
the document in memory in the form of a succinct tree data-structure
(based for instance on balanced parenthesis: a survey of
the most popular succinct tree representations can be found in
\cite{Gonzalo10}). The final data-structure (e.g.,  a DOM
representation) of the document can then be built from the temporary
one, by replaying a sequence of SAX events while
traversing the temporary data-structure and by not synthesizing events
for pruned sub-trees. An alternative solution is to store on disk the
sequence of SAX events and process it backward, thus simulating a
bottom-up evaluation (validation of regular tree grammars and therefore
projection can be done in a deterministic bottom-up fashion). Such
a technique was used in \cite{koch03} to efficiently evaluate node
selecting queries bottom-up on documents up to 1 GB of size.



==> introduction.tex <==
% Master File: main.tex
\section{Introduction}
\label{sec:intro}

%As explained by Marian and Sim\'eon~\cite{amelieVLDB}, 
Main-memory XML
query engines are often the primary choice for applications that do
not wish or cannot afford to build secondary storage indexes or load a
database before query processing. One of the main optimisation
techniques recently adopted in this context is XML data projection (or
pruning)~\cite{amelieVLDB,annaDatax}. 

% 
% Main memory XML querying
% systems \cite{what??} are the only feasible solution in several
% kind of applications.
% 
% , typically in those  that cannot or do not
% want to create and manage secondary memory  indexes, or, more in
% general, want any kind of heavy data processing before
% querying. \dario{Here it would be fine to find examples...probably
%   we should give a look at Galax web page.}\beppe{No, cut instead}
% 

The basic idea  behind document projection is
very simple and powerful at the same time. Given a
query $Q$ over  a document $D$, sub-trees of $D$ that are not necessary to
evaluate $Q$ are pruned, thus yielding a smaller document $D'$. Then
$Q$ is executed over $D'$, hence avoiding to allocate and process nodes
that will never be reached by navigational specifications in $Q$. This
ensures that evaluation over $D'$ is equivalent to and more efficient
than the evaluation over $D$.




As shown in \cite{amelieVLDB,annaDatax}, XML navigation
specifications expressed in queries tend to be very selective,
especially in terms of document structure. Therefore, pruning
may yield  significant improvements both in terms of execution time and in terms of
memory usage: as a matter of facts, for main-memory XML query engines,  very
large documents can not be queried without pruning.


\subsection{State of the art}
Marian and Sim\'eon~\cite{amelieVLDB} propose that  the actual
data-needs of an XQuery query $Q$ 
%
%\beppe{Here we have to say which languages $Q$ may belong to}
%
(that is, the
part of data that is necessary to the execution of the query) is
determined by statically extracting all paths in $Q$. These paths
are then applied to $D$ at load time, in a SAX-event based fashion,
in order to prune unneeded parts of data. The technique is powerful
since: $(i)$ it applies to most of XQuery \emph{core}, $(ii)$ it can
be applied to a set of queries over the same document, and $(iii)$
it does not require any \emph{a priori} knowledge of the structure of $D$.
However, this technique suffers some limitations. First, the
document loader-pruner can manage neither
\emph{backward axes} nor path expressions with predicates (sometimes
called ``qualifiers'') which, especially the latter, can
contain precious information to optimise pruning. 
Second, the advantage described in point $(iii)$ becomes a big drawback when ``\dos'' occur in paths since, in that case, the technique does not behave efficiently
in terms of loading time and pruning precision (hence, memory
allocation). Indeed, when a \dos
 is present in a projection path, the pruning process requires 
to visit all descendants of a node in order to decide whether the node
contains a useful descendant. What is worst is that pruning time tends
to be quite high and it drastically increases (together with memory
consumption) when the number of \dos
augments in the pruning path-set. As a matter of fact, in this
technique, pruning corresponds to computing a further query whose time
and memory occupation may be comparable to those required to compute
the original query. In particular, in this technique every occurrence
of  \dos may yield a full exploration of the tree 
(e.g., see in \cite{amelieVLDB} the test for the XMark~\cite{xmark}
query Q7 which only contains three \dos steps and for which
just computing the pruning takes longer than executing the query on
the original document).
Therefore, 
pruning execution overhead and its high memory footprint may
jeopardise the gains obtained by using the
pruned document. Third and finally, as we
explain in Section~\ref{sec:xquery}, the precision of pruning drastically
degrades (down to being nullified) for queries containing the XPath expressions  
\descendant[\textit{node\!\!}]\filt{\textit{cond}}, which are very useful
and used in practice.

Bressan \textit{et al.\ }\cite{annaDatax} introduce a different and quite
precise XML pruning technique for a subset of XQuery FLWR
expressions. The technique is
based on the \emph{a priori} knowledge of a data-guide for $D$. The
document $D$ is first matched against an abstract representation of $Q$.
Pruning is then performed at run time, it is very precise, and, thanks
to the use of some indexes over the data-guide, it ensures good
improvements in terms of query execution time. However, the
technique is one-query oriented---in the sense that it cannot be
applied to multiple queries---, it does not handle XPath predicates, and cannot
handle backward axes
(recall that the encodings of~\cite{omfb2002}  are defined for XPath, and no
extension to XQuery-like languages is known). Also, the approach
requires the construction and management of the data-guide and
of adequate indexes.

%%%\kim{RajoutÃ© le related work suivant:}

Motivated by efficient XML stream processing, Green \textit{et al.}~\cite{gupta}
introduced a framework for discarding sequences of SAX
events in an XML data stream. Although their approach allows them to
prune an input stream with respect to sets of queries, the language they
handle is restricted to forward linear XPath expressions (that is,
XPath expressions with only \child and \descendant axes and without
predicates).


\subsection{Our contribution}
In this article, we present  a new pruning  approach that is applicable
in the presence of typed XML data. This is often the case,  as most
applications require that data are valid with respect to some external schema
(e.g., {\sc Dtd}~\cite{dtd} or XML Schema~\cite{xmlschema}).


Our technique combines the advantages of the previously mentioned works
while relaxing their limitations. Unlike
\cite{amelieVLDB,annaDatax,gupta}, our approach accounts for  backward axes, performs a fine-grained analysis of predicates,  allows  (unlike \cite{annaDatax}) for dealing with bunches of
queries, and (unlike \cite{amelieVLDB}) cannot be jeopardised by pruning overhead.  Our solution provides in all cases comparable or greater
precision than the other approaches, while it requires always negligible
or no pruning overhead. Moreover, contrary
to~\cite{amelieVLDB,annaDatax}, our approach is formally proved to be
{\it sound\/} (i.e., pruning does not alter the result of que\-ries) and,
furthermore, we can also prove it to be {\it complete\/} (i.e.,  it
produces the best possible type-driven pruning) for a
substantial class of queries and {\sc dtd}s.


For the sake of presentation we introduce our framework in three steps. In the first step, we consider a simplified
version of XPath, we dub XPath$^\ell$, which includes only
upward/downward axes and unnested disjunctive predicates. We define for XPath$^\ell$
a static analysis that determines a set of type names, a \textit{type
  projector\/}, that is then used to prune the document(s). One of the
particular features of this approach is that our pruning algorithm is characterised by a constant (and low) memory consumption and by an execution time linear in the size of the document to prune. More precisely, a pruning based on type projectors is equivalent to a single buffer-less one-pass traversal of the parsed document (it simply
discards elements not generated by any of the names in the
projector). So if embedded in query processors, pruning can be executed during parsing and/or validation and brings no overhead at all, while
if used as an external tool it requires a time always smaller than or
equal to the time used to parse the queried document. Soundness and (partial)
completeness results for the static analysis are stated.

The second step consists of extending the analysis to the whole XPath 
(more precisely, to XPath 1.0),
that is, we need to show how to deal with  missing axes and with general
predicates as defined in the XPath specification. This is done by
associating to each XPath query $Q$ a XPath$^\ell$ query $P$ that
soundly approximates $Q$, in the sense that the projector inferred for
$P$ by the static analysis developed at the first step is also a sound projector for $Q$.


The final step of our process is to extend the approach to XQuery (hence, to XPath 2.0). This is obtained in the same way as done in~\cite{amelieVLDB}, by
defining a path extraction algorithm. Our
path extraction algorithm improves and extends in several aspects (in particular, in terms of
extracted paths' selectivity) the one of~\cite{amelieVLDB}. It also
computes the XPath$^\ell$ approximation of the extracted paths so that
the static analysis of the first step can be directly applied to them.

 We  prove some important closure properties that guarantee that 
type projections can always be performed at load time during the validation process,
and this without any overhead. In particular for XML documents typed with \dtd{s} or XML Schemas 
the document can be pruned in streaming. 

We gauged and validated our approach by testing it both on the
XPathMark~\cite{xpathmark} and on the XMark~\cite{xmark}
benchmarks. The result of this validation confirmed what was expected: thanks to the
handling of backward axes and of predicates the precision of our pruning is
in general noticeably higher than that of current approaches; the pruning
time is linear in the size of the queried document and has a very low memory footprint; the time of the static
analysis is always negligible (lower than half a second on the hardware we used for our benchmarks described in Section~\ref{sec:experiments}) even for
complex queries and \dtd{s}. But benchmarks also brought unexpected (and
quite pleasant) results. In particular, they showed that type-based pruning brings
benefits that go beyond those of the reduced size of the pruned
document: by excluding a whole set of data structures (those whose type
names are not included in the type projector), the pruning may
drastically reduce the resources that must be allocated at run-time by
the query processor. For instance, our benchmarks show that for several
XMark and XPathMark queries our pruning yields a document whose size is two thirds of the size
of the original document, but the query can then be processed using three
times less memory than when processed on the original document. This is
a very important gain, especially for DOM-based processors, or memory
sensitive processors. 
Not only our approach is relevant in the case of main memory query engines such as Saxon but it is also shown to be useful for native query engines as efficient as MonetDB~\cite{bonea06}. Even in the latter case our experiments demonstrate the relevance of type projection as a complementary optimisation technique. Indeed, this not totally surprising as type projection can be thought of as a way of defining clustering policies in the same line as what was done in the context of object-oriented databases~\cite{o2bookcl,Benzaken90b,Benzakenetal90a}. Clustering and indexing are well-known complementary tools used in the context of query optimisation.
%% \vero{Idid it see upper}
%% \beppe{I would add here a sentence for
%%   MonetDB. E.G. The benchmarks also showed that our pruning technique
%%   dramatically increase efficiency even in case of engines, such as
%%   MonetDB, that work on native XML data and store in main memory only
%%   indexes to the data. What is relatively surprising here is the
%%   amount of the gain obtained with these system. It is just relatively
%%   surprising, however, since, as a matter of facts, our projectors
%%   implements an efficient clustering policy similar to the one defined
%%   by Véronique Benzaken~\cite{} for the O$_2$ OODBMS~\cite{} VERO
%%   RISCRIVI!!}
%% \kim{Looks good to me now}

As an aside we want to stress that our technique relies on the definition of a
new type system for XPath able to handle backward axes which, alone on
its own, constitutes a contribution of this work. In particular the
precision  of type inference for backward axes goes beyond what is proposed in the XQuery
Static Semantic recommendation (\cite{XQuerysem}).



Finally, we presented a preliminary version of this work at the VLDB 2006 conference~\cite{BCCN06}. The 
work in this article, besides including full proofs and having been
cleaned up, improves and extends the work in~\cite{BCCN06} in several important
aspects. First and foremost we generalized the definition of type
projectors by using as projectors sets of production rules (as opposed to the sets
of non-terminals used in~\cite{BCCN06}) of regular tree grammars (as opposed to the
\dtd{s} used in~\cite{BCCN06}).
This generalization was far from being straightforward. In particular,  we had to  prove the applicability 
of our technique to the more general framework under consideration (cf.\ Section~\ref{ssec:closure}). However the result is  worth the
effort since the advantages of this generalization are twofold. On the one hand using  
regular tree grammars allows us to
compute type projectors for every kind of XML
schema formalism we are aware of as, for instance, \dtd{s}, XMLSchemas, \cduce{}
and XDuce types, Relax-Core and TREX schemas. On the other hand, inferring
grammar production rules rather than grammar non-terminals allows
us to compute context-aware and, thus, more precise projectors. More precisely,
the new type projectors introduced in this work
can prune a subtree not only based on its tag (as it was done in~\cite{BCCN06}),
but also on any structural condition expressible by a regular tree language. So for instance
our pruning process may decide to prune just one of two trees
generated by the same non-terminal, because they appear in different contexts
(in~\cite{BCCN06} either both trees were pruned or they were both preserved).
Therefore these new projectors are both more general and 
can perform much finer-grained pruning. Second,
although we develop the theory of type projection for a
simplified data-model and restricted forms of XPath expressions, we
thoroughly detail how to tackle many of the peculiarities of the XML
and XPath specifications \cite{xml:spec,xpath:spec}, including the
handling of attributes, the presence of absolute axes in XPath
predicates or a wide range of predefined XPath functions (all absent in~\cite{BCCN06}). 
The path language we formally
study  extends the one in~\cite{BCCN06} with top-level unions of
paths, predicate conjunctions (``\texttt{and}'') and arbitrarily nested
predicates (our previous work formally treated only non-nested
predicates and resorted to an approximation in the case of nested
predicates).
Third, we provide an extensive list of experiments showing the
overall benefits of type projection for a wide range of queries and
query engines. These experiments supersede the early benchmarks
realised in \cite{BCCN06} and show that despite the advances in XML
query technologies in the recent years, our static analysis can
significantly improve the performances (both in time and memory consumption)
of many different XML query engines.

 

\subsection{Plan of the article}
%\beppe{TO BE REWRITTEN}\vero{DONE}
The article is organised as follows. Section~\ref{sec:notations} introduces
basic definitions and notations: data model, types, validation. Section~\ref{sec:typeproj} presents type projectors, type-based projection, and several theoretical (closure) properties. In Section~\ref{sec:xpathell} we define
XPath$^\ell$ and its semantics, and formally describe how general XPath
predicates can be soundly approximated in it. In Section~\ref{sec:staticanalysis} we
present our type projectors inference algorithm for XPath$^\ell$ and state
its formal properties. In Section~\ref{sec:fullxpath} we extend our approach to full XPath and in
Section~\ref{sec:xquery} to
XQuery. In Section~\ref{sec:extother} we discuss how to apply our technique to other typing policies as well as to un-typed documents. Section~\ref{sec:experiments} presents our implementation and reports the
results of our benchmarks. We finally conclude in Section~\ref{sec:conclusion} by
presenting the perspectives of this work. Last, for the sake of clarity, all the proofs for the stated results are given in Appendix~\ref{sec:appendix}.

% \ifWithProofs
% An appendix contains the proofs not included in the main text.
% \else

% For space reasons all proofs of properties are omitted from this presentation. They can
% be found in the extended version of this work.
% \fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 




==> packages.tex <==
\usepackage[utf8x]{inputenc}
\usepackage[british]{babel}
\usepackage{ifthen}
%% T5 is for vietnamese
\usepackage[T5,T1]{fontenc}
\usepackage{xspace}
\usepackage{color}
\usepackage{amssymb,amsmath}
\usepackage{url}
\usepackage{stmaryrd}
\usepackage{calc}
\usepackage{framed}
\usepackage{bm}
\usepackage{bussproofs}
\usepackage{alltt}
\usepackage{graphicx}
%%% required by the journal style
\usepackage{mathptmx}
%%% i nostri hack personali
%%%\usepackage{macros}

\usepackage{ifthen}
\newboolean{withproofs}
%% change to true to have the proofs in the text
\setboolean{withproofs}{false}
\ifthenelse{\boolean{withproofs}}{
\newenvironment{comment}{}{}}{
\usepackage{verbatim}}

